An algebraic multigrid method for $Q_2-Q_1$ mixed discretizations of the Navier-Stokes equations

Algebraic multigrid (AMG) preconditioners are considered for discretized systems of partial differential equations (PDEs) where unknowns associated with different physical quantities are not necessarily co-located at mesh points. Specifically, we investigate a $Q_2-Q_1$ mixed finite element discretization of the incompressible Navier-Stokes equations where the number of velocity nodes is much greater than the number of pressure nodes. Consequently, some velocity degrees-of-freedom (dofs) are defined at spatial locations where there are no corresponding pressure dofs. Thus, AMG approaches leveraging this co-located structure are not applicable. This paper instead proposes an automatic AMG coarsening that mimics certain pressure/velocity dof relationships of the $Q_2-Q_1$ discretization. The main idea is to first automatically define coarse pressures in a somewhat standard AMG fashion and then to carefully (but automatically) choose coarse velocity unknowns so that the spatial location relationship between pressure and velocity dofs resembles that on the finest grid. To define coefficients within the inter-grid transfers, an energy minimization AMG (EMIN-AMG) is utilized. EMIN-AMG is not tied to specific coarsening schemes and grid transfer sparsity patterns, and so it is applicable to the proposed coarsening. Numerical results highlighting solver performance are given on Stokes and incompressible Navier-Stokes problems.

==> ack.tex <==
% Funding and grants.
% Try follow http://science.energy.gov/funding-opportunities/acknowledgements/
\fix[inline]{AP}{The paragraph needs fixing}
This material is based upon work supported by the U.S. Department of Energy (DOE), Office of Science, Office of Advanced Scientific Computing Research (ASCR).
This research was supported in part by \ldots.
%
% Any paper with a Sandia author needs the following funding statement.
%
Sandia National Laboratories is a multiprogram laboratory managed and
operated by Sandia Corporation, a wholly owned subsidiary of Lockheed
Martin Corporation, for the DOE's National Nuclear Security
Administration under contract DE--AC04--94AL85000.


==> fig/fig2tikz <==
#!/usr/bin/env python
import fig, sys, math, optparse

# FIXME: arrow colors (regression)
# TODO (good test figure: lemma1.fig):
# - tolerance parameter
#   * for grouping identical coordinates
#   * for detecting points on a circle
# - recognize node labels (i.e. text near a circular node)
# - only convert small circles into nodes

_latexChars = {
	'^':  r"{\textasciicircum}",
	'~':  r"{\textasciitilde}",
	'\\': r"{\textbackslash}",
	'|':  r"{\textbar}",
	'<':  r"{\textless}",
	'>':  r"{\textgreater}",
	'\"': r"{\textquotedblright}",
	}

# TODO: double-check and extract numbers from texmf/tex/latex/base/size1[012].clo
_latexFontSizes = {
	5: "tiny",
	7: "scriptsize",
	8: "footnotesize",
	9: "small",
	10: "normalsize",
	12: "large",
	14: "Large",
	18: "LARGE",
	20: "huge",
	24: "Huge",
	}

def escapeLaTeX(s):
	result = ""
	for ch in s:
		if ch in "$%_{}&#":
			result += r'\%s' % ch
		elif ch in r'^~\|<>"':
			result += _latexChars[ch]
		else:
			result += ch
	return result

def latexFloat(num, fractDigits = 5):
	result = ("%%20.%df" % fractDigits) % num
	b = 0
	while result[b] == " ":
		b += 1
	e = len(result)
	while result[e-1] == "0":
		e -= 1
	if result[e-1] == ".":
		e -= 1
	return result[b:e]

# --------------------------------------------------------------------

_arrowMapping = {
	fig.arStick  : 'to',
	fig.arClosed : 'triangle 45',
	fig.arClosedIndented : 'stealth',
	fig.arClosedPointed : 'diamond',
	}

_capStyleMapping = {
	fig.capStyleButt : 'butt',
	fig.capStyleRound : 'round',
	fig.capStyleProjecting : 'rect',
	}

_joinStyleMapping = {
	fig.joinStyleMiter : 'miter',
	fig.joinStyleBevel : 'bevel',
	fig.joinStyleRound : 'round',
	}

_colorMapping = {
	fig.colorBlack : 'black',
	fig.colorBlue : 'blue',
	fig.colorGreen : 'green',
	fig.colorCyan : 'cyan',
	fig.colorRed : 'red',
	fig.colorMagenta : 'magenta',
	fig.colorYellow : 'yellow',
	fig.colorWhite : 'white',
	}

_fillStyleMapping = {
# 	fig.fillStyleLeft30 : "",
# 	fig.fillStyleRight30 : "",
# 	fig.fillStyleCrossed30 : "",
	fig.fillStyleLeft45 : "north west lines",
	fig.fillStyleRight45 : "north east lines",
 	fig.fillStyleCrossed45 : "crosshatch",
	fig.fillStyleHorizontalBricks : "bricks",
# 	fig.fillStyleVerticalBricks : "",
	fig.fillStyleHorizontalLines : "horizontal lines",
	fig.fillStyleVerticalLines : "vertical lines",
	fig.fillStyleCrosshatch : "grid",
# 	fig.fillStyleHorizontalShingles1 : "",
# 	fig.fillStyleHorizontalShingles2 : "",
# 	fig.fillStyleVerticalShingles1 : "",
# 	fig.fillStyleVerticalShingles2 : "",
# 	fig.fillStyleFishScales : "",
# 	fig.fillStyleSmallFishScales : "",
# 	fig.fillStyleCircles : "",
# 	fig.fillStyleHexagons : "",
# 	fig.fillStyleOctagons : "",
# 	fig.fillStyleHorizontalTireTreads : "",
# 	fig.fillStyleVerticalTireTreads : "",
	}

def arrowCode(arrow):
	if not arrow:
		return ""
	result = _arrowMapping[arrow.type]
	if arrow.style == fig.asHollow and result in (
		"triangle 45", "diamond"):
		result = "open " + result
	return result

class Options(list):
	def __setitem__(self, key, value):
		if isinstance(key, int):
			list.__setitem__(self, key, value)
		else:
			for i, (existing, _) in enumerate(self):
				if key == existing:
					del self[i]
					break
			self.append((key, value))

	def __getitem__(self, index):
		if isinstance(index, int):
			list.__getitem__(self, index)
		else:
			for key, value in self:
				if key == index:
					return value
			raise KeyError("Option '%s' not set!" % index)

	def __delitem__(self, index):
		if isinstance(index, int):
			list.__delitem__(self, index)
		else:
			for i, (existing, value) in enumerate(self):
				if index == existing:
					list.__delitem__(self, i)
					return
			raise KeyError("Option '%s' not set!" % index)

	def __str__(self):
		if not self:
			return ""
		result = []
		for key, value in self:
			if value:
				if key in ("style", "color"):
					result.append(value)
				else:
					result.append("%s=%s" % (key, value))
			else:
				result.append(key)
		return "[%s]" % (",".join(result), )

	def get(self, key, default):
		for existing, value in self:
			if existing == key:
				return value
		return default

	def __contains__(self, key):
		for existing, value in self:
			if existing == key:
				return True
		return False

	def append(self, option):
		if isinstance(option, str):
			list.append(self, (option, None))
		else:
			assert len(option) == 2
			list.append(self, option)

class TikZConverter(object):
	def __init__(self, figFile, outFile, includeBaseDir = ""):
		self.figFile = figFile
		self.outFile = outFile
		if figFile.metric:
			# if metric, 450 units is 1cm (in the default ppi setting of 1200)
			self.scale = 8./3./figFile.ppi
		else:
			self.scale = 2.54/figFile.ppi # number from tneumann's fig2pgf
		self.fontMag = self.figFile.magnification / 100.0

		self.includeBaseDir = includeBaseDir
		self.useTextNodes = True
		self.textAnchor = "base"
		self.splinesAsPolylines = True
		self.detectClosing = True
		self.detectNodes = False
		self.maxNodeRadius = fig.unitCM
		self.connectTolerance = None
		self.logicalThickness = True
		self.defineYAxis = True

		self._circleNodeCount = 0
		self._nodePositions = {}
		self._definedColors = {}
		self._warned = {}

	def _warnOnce(self, message):
		if not message in self._warned:
			self._warned[message] = True
			sys.stderr.write("WARNING: %s\n" % message)

	def coordinate(self, xy):
		"""xy should be a fig coordinate (fig.Vector) to be converted
		to a TikZ coordinate (returned as str)."""

		named = self._nodePositions.get(tuple(xy), None)
		if named:
			return "(%s)" % named
		elif self.connectTolerance:
			nearest = (self.connectTolerance, None)
			for pos in self._nodePositions.keys():
				if xy.dist(pos) < nearest[0]:
					nearest = (xy.dist(pos), pos)
			if nearest[1]:
				return "(%s)" % self._nodePositions[nearest[1]]

		x = xy[0]
		y = xy[1]
		if not self.defineYAxis:
			y = -y
		return "(%s,%s)" % (latexFloat(x*self.scale),
							latexFloat(y*self.scale))

	def dimensionCM(self, length):
		return "%scm" % latexFloat(length*self.scale)

	def figPt(self, figPt):
		return "%sbp" % latexFloat(figPt*72./80, 1)

	def getNode(self, circle): # TODO: allow other objects
		if not self.detectNodes:
			return None
		if circle.radius[0] > self.maxNodeRadius:
			return None
		self._circleNodeCount += 1 # TODO: allow unnamed nodes
		name = "circle%d" % self._circleNodeCount
		self._nodePositions[tuple(circle.center)] = name
		return name

	def writePicture(self):
		options = Options()
		if self.optimalAppearance:
			options.append("even odd rule")

		if self.defineYAxis:
			options["y"] = "-1cm"

		self.outFile.write("\\begin{tikzpicture}%s\n" % options)

		if self.detectNodes:
			self.outFile.write("\n% circle nodes:\n")
			circles = self.figFile.findObjects(type = fig.Circle)
			for circle in circles:
				if self.writeCircleNode(circle):
					self.figFile.remove(circle) # don't output twice

		for depth in reversed(self.figFile.layers()):
		  self.outFile.write("\n%% objects at depth %d:\n" % depth)
		  for o in self.figFile.layer(depth):
			if self.detectClosing and isinstance(o, fig.Polyline):
				if o.points[-1] == o.points[0]:
					o.changeType(fig.ptPolygon)
					if len(o.points) == 4:
						bb = o.bounds()
						isRect = True
						for p in o.points:
							if p[0] not in (bb.x1, bb.x2) or \
							   p[1] not in (bb.y1, bb.y2):
								isRect = False
						if isRect:
							o.changeType(fig.ptBox)
			if o.comment:
				c = o.comment.rstrip()
				self.outFile.write("%%%s\n" % c.replace("\n", "\n%"))
			if isinstance(o, fig.ArcBase):
				self.writeArcBase(o)
			elif isinstance(o, fig.Circle):
				self.writeCircle(o)
			elif isinstance(o, fig.EllipseBase):
				self.writeEllipseBase(o)
			elif type(o) == fig.PictureBBox:
				self.writePictureBBox(o)
			elif isinstance(o, fig.ArcBox):
				self.writeArcBox(o)
			elif isinstance(o, fig.PolyBox):
				self.writePolyBox(o)
			elif isinstance(o, fig.PolylineBase):
				self.writePolylineBase(o)
			elif isinstance(o, fig.SplineBase):
				self.writeSplineBase(o)
			elif isinstance(o, fig.Text):
				if self.useTextNodes:
					self.writeTextNode(o)
				else:
					self.writeText(o)
			else:
				self._warnOnce("%s objects not yet supported!" % type(o))

		self.outFile.write("\n\\end{tikzpicture}%\n")

	def defineColor(self, name, figColor):
		if figColor in _colorMapping:
			return _colorMapping[figColor]

		r, g, b = self.figFile.colorRGB(figColor)
		if self._definedColors.get(name, None) != (r,g,b):
			if r == g == b:
				self.outFile.write(
					"\\definecolor{%s}{gray}{%s}\n" % (name, latexFloat(r/255.)))
			else:
				self.outFile.write(
					"\\definecolor{%s}{rgb}{%s,%s,%s}\n" %
					(name, latexFloat(r/255.), latexFloat(g/255.), latexFloat(b/255.)))
			self._definedColors[name] = (r,g,b)
		return name

	def tikzOptions(self, object):
		options = Options()

		if object.lineWidth:
			if object.penColor != fig.colorDefault:
				penColor = self.defineColor("penColor", object.penColor)
				options["draw"] = penColor
			else:
				options["draw"] = None

			if object.lineWidth > 1:
				if self.logicalThickness and object.lineWidth <= 5:
					options.append(("semithick", "thick", "very thick", "ultra thick")[object.lineWidth-2])
				else:
					options["line width"] = self.figPt(object.lineWidth-1)
			if object.capStyle != fig.capStyleButt:
				options["cap"] = _capStyleMapping[object.capStyle]
			if object.joinStyle != fig.joinStyleMiter:
				options["join"] = _joinStyleMapping[object.joinStyle]

		if object.fillStyle != fig.fillStyleNone:
			pattern = ""
			fillColor = None
			if object.fillColor != fig.colorDefault:
				if object.fillColor == object.penColor and object.lineWidth:
					fillColor = penColor
				else:
					fillColor = self.defineColor("fillColor", object.fillColor)

			if object.fillStyle == fig.fillStyleSolid:
				pass
			elif object.fillStyle < fig.fillStyleSolid:
				if not fillColor or fillColor == "black":
					fillColor = "black!%s" % (object.fillStyle*5)
				else:
					fillColor += "!%d!black" % (object.fillStyle*5)
			elif object.fillStyle <= fig.fillStyleWhite:
				if fillColor in ("black", "white", None):
					self._warnOnce("fill style %s with %s fill color should not happen!" % (object.fillStyle, fillColor or "default"))
				fillColor += "!%d" % (100 - (object.fillStyle - fig.fillStyleSolid)*5)
			elif object.fillStyle in _fillStyleMapping:
				pattern = _fillStyleMapping[object.fillStyle]
			else:
				self._warnOnce("fill style %s not yet supported!" % object.fillStyle)

			if fillColor is not None and fillColor == options.get("draw", False):
				options["draw"] = None
				options["fill"] = None
				options["color"] = fillColor
			else:
				options["fill"] = fillColor

			if pattern:
				options["pattern"] = pattern

		if object.lineStyle == fig.lineStyleDotted:
			options["style"] = "dotted"
		elif object.lineStyle == fig.lineStyleDashed:
			options["style"] = "dashed"
		elif object.lineStyle not in (fig.lineStyleDefault, fig.lineStyleSolid):
			# TODO style=solid in TikZ?
			self._warnOnce("line style %s not yet supported!" % object.lineStyle)

		if object.forwardArrow or object.backwardArrow:
			options["arrows"] = "%s-%s" % (
				arrowCode(object.backwardArrow),
				arrowCode(object.forwardArrow))

		# simplifications:
		if "draw" in options and not "fill" in options:
			# \path[draw=black] -> \path[draw,color=black] {.. \draw[black] }
			if options["draw"] is not None:
				options["color"] = options["draw"]
			options["draw"] = None # should become \draw

		return options

	def pathIntro(self, object, options = None):
		if not options:
			options = self.tikzOptions(object)
		else:
			options.extend(self.tikzOptions(object))

		command = ""
		if options.get("draw", False) is None:
			command = "draw"
			del options["draw"]
		if options.get("fill", False) is None:
			command = "fill" + command
			del options["fill"]

		if not command:
			command = "path"
			#return "%"
		return "\\%s%s" % (command, options)

	def writeArcBase(self, arc):
		a1, a2 = arc.angles()
		startPoint = 0

		a1 = int(round(math.degrees(a1)))
		a2 = int(round(math.degrees(a2)))
		if a2 >= 360:
			temp = a1
			a1 = a2 - 360
			a2 = temp - 360
			startPoint = 2
		elif a2 <= -360:
			temp = a1
			a1 = a2 + 360
			a2 = temp + 360
			startPoint = 2

		if startPoint:
			arc.forwardArrow, arc.backwardArrow = \
							  arc.backwardArrow, arc.forwardArrow

		draw = cycle = ""
		if arc.closed():
			draw = "-- "
			cycle = " -- %s -- cycle" % self.coordinate(arc.center)

		if self.defineYAxis:
			a1 = -a1
			a2 = -a2
		self.outFile.write("%s %s %s+(%s:%s) arc (%s:%s:%s)%s;\n" % (
			self.pathIntro(arc),
			self.coordinate(arc.center),
			draw, a1, latexFloat(arc.radius()*self.scale),
			a1, a2,
			latexFloat(arc.radius()*self.scale),
			cycle))

	def writeEllipseBase(self, ellipse):
		# TODO: ellipse.angle
		self.outFile.write("%s %s ellipse (%s and %s);\n" % (
			self.pathIntro(ellipse),
			self.coordinate(ellipse.center),
			self.dimensionCM(ellipse.radius[0]),
			self.dimensionCM(ellipse.radius[1])))

	def writeCircleNode(self, circle):
		center = self.coordinate(circle.center)
		node = self.getNode(circle)
		if not node:
			return
		options = self.tikzOptions(circle)
		options.insert(0, ("circle", None))
		if node: # named node?
			node = " (%s)" % node
		options["minimum size"] = self.dimensionCM(circle.radius[0]*2)
		self.outFile.write("\\node%s at %s%s {};\n" % (
			options, center, node))
		return node

	def writeCircle(self, circle):
		center = self.coordinate(circle.center)
		self.outFile.write("%s %s circle (%s);\n" % (
			self.pathIntro(circle), center,
			self.dimensionCM(circle.radius[0])))

	def writePolylineBase(self, poly):
		path = " -- ".join(map(self.coordinate, poly.points))
		if poly.closed():
			path += " -- cycle"
		self.outFile.write(
			"%s %s;\n" % (self.pathIntro(poly), path))

	def writeSplineBase(self, spline):
		if not spline.closed() and len(spline.points) == 3:
			self.outFile.write(
				"%s %s .. controls %s .. %s;\n" % (
				(self.pathIntro(spline), ) + tuple(
				map(self.coordinate, spline.points))))
			return

		if self.splinesAsPolylines:
			return self.writePolylineBase(spline)
		else:
			self._warnOnce("X-splines cannot be 100% correctly converted!")

		self.outFile.write(self.pathIntro(spline))

		cycle = spline.closed() and " cycle" or ""

		self.outFile.write(" plot[smooth%s] coordinates {%s};\n" % (
			cycle, " ".join(map(self.coordinate, spline.points))))

	def writePolyBox(self, polyBox):
		self.outFile.write("%s %s rectangle %s;\n" % (
			self.pathIntro(polyBox),
			self.coordinate(polyBox.points[0]),
			self.coordinate(polyBox.points[2])))

	def writeArcBox(self, arcBox):
		self.outFile.write("%s %s rectangle %s;\n" % (
			self.pathIntro(arcBox, options = Options([
			("rounded corners", self.figPt(arcBox.radius))])),
			self.coordinate(arcBox.points[0]),
			self.coordinate(arcBox.points[2])))

	def writePictureBBox(self, pictureBBox):
		nodeOptions = Options()
		nodeOptions["anchor"] = "north west"
		nodeOptions["inner sep"] = "0pt"

		self.outFile.write("\\node%s at %s {\\includegraphics[width=%s,height=%s]{%s%s}};\n" % (
			nodeOptions,
			self.coordinate(pictureBBox.bounds().upperLeft()),
			self.dimensionCM(pictureBBox.bounds().width()),
			self.dimensionCM(pictureBBox.bounds().height()),
			self.includeBaseDir,
			pictureBBox.filename))

	def _textSizeCommand(self, text):
		result = ""

		texSize = text.fontSize
		if not text.fontFlags & fig.ffRigid:
			texSize *= self.fontMag

		if texSize: # TODO: allow setting e.g. fontMag to 0 to prevent this:
			if texSize in _latexFontSizes: # TODO: switchable, 12pt support
				if texSize != 10:
					result = r"\%s{}" % (_latexFontSizes[texSize], )
			else:
				baselineSkip = texSize * 1.2
				result = r"\fontsize{%s}{%s}\selectfont{}" % (
					texSize, baselineSkip, )

		return result

	def _textInFont(self, text):
		if text.font == fig.fontZapfDingbats:
			# FIXME: \usepackage{pifont}
			result = "".join([r"\ding{%d}" % ord(ch) for ch in text.text])
		elif text.fontFlags & fig.ffSpecial:
			result = text.text
		else:
			result = escapeLaTeX(text.text)

		if text.fontFlags & fig.ffPostScript:
			pass # TODO
		else:
			if text.font == fig.fontLaTeXDefault:
				pass
			elif text.font == fig.fontLaTeXRoman:
				result = r"\rmfamily " + result
			elif text.font == fig.fontLaTeXBold:
				result = r"\bfseries " + result
			elif text.font == fig.fontLaTeXItalic:
				result = r"\itshape " + result
			elif text.font == fig.fontLaTeXSansSerif:
				result = r"\sffamily " + result
			elif text.font == fig.fontLaTeXTypewriter:
				result = r"\ttfamily " + result

		return result

	def writeText(self, text):
		if text.fontFlags & fig.ffHidden:
			return

		options = ["base"]

		if text.alignment == fig.alignLeft:
			options.append("left")
		elif text.alignment == fig.alignRight:
			options.append("right")

		if text.pos[0]:
			options.append("x=%s" % self.dimensionCM(text.pos[0]))
		if text.pos[1]:
			options.append("y=%s" % self.dimensionCM(-text.pos[1]))
		if text.angle:
			options.append("rotate=%s" % round(math.degrees(text.angle)))

		str = self._textInFont(text)

		if text.penColor != fig.colorDefault:
			textColor = self.defineColor("textColor", text.penColor)
			str = r"\color{%s}%s" % (textColor, str)

		self.outFile.write("\\pgftext[%s]{%s%s}\n" % (
			",".join(options),
			self._textSizeCommand(text), str))

	def writeTextNode(self, text):
		if text.fontFlags & fig.ffHidden:
			return

		options = Options()
		nodeOptions = Options()

		if text.penColor != fig.colorDefault:
			nodeOptions["text"] = self.defineColor("textColor", text.penColor)

		anchor = self.textAnchor
		if text.alignment == fig.alignLeft:
			anchor += " west"
		elif text.alignment == fig.alignRight:
			anchor += " east"
		nodeOptions["anchor"] = anchor

		if text.angle:
			nodeOptions["rotate"] = round(math.degrees(text.angle))

		str = self._textInFont(text)

		self.outFile.write("\\path%s %s node%s {%s%s};\n" % (
			options,
			self.coordinate(text.pos), nodeOptions,
			self._textSizeCommand(text), str))

# --------------------------------------------------------------------

op = optparse.OptionParser(usage="%prog [options] foo.fig > foo.tikz")
op.add_option("-a", "--appearance", action = "store_true",
			  dest = "appearance", default = False,
			  help = "optimize for most similar appearance at the price of more verbose code (default: off)")
op.add_option("-b", "--basedir", action = "store",
			  dest = "baseDir", default = "", metavar = "IMAGEDIR/",
			  help = "path prefix that is directly prepended before image filenames (use this if you \\input the TikZ code from another directory)")
op.add_option("-y", "--yaxis", action = "store_false",
			  dest = "defineYAxis", default = True,
			  help = "don't redefine Y axis (default: use y=-1cm for more natural coordinates within TikZ code)")
op.add_option("--anchor", action = "store",
			  dest = "textAnchor", default = "base",
			  help = "vertical anchor, one of 'base', 'center', 'north', 'south' (default: base)")
op.add_option("-f", "--nofonts", action = "store_true",
			  dest = "nofonts", default = False,
			  help = "do not output fontsize commands")
op.add_option("--detectnodes", action = "store_true",
			  dest = "detectNodes", default = False,
			  help = "try to recognize graphs and connect named nodes (only circles ATM)")
op.add_option("--scale", metavar = "FACTOR",
			  dest = "scale", default = 1.0, type = "float",
			  help = "scale whole figure by the given factor")
op.add_option("--splines", metavar = "lines|plot",
			  dest = "splines", default = "lines",
			  help = "convert X-splines into polygonal lines (default) or smooth plots")
# op.add_option("-t", "--textnodes", action = "store_true",
# 			  dest = "textNodes", default = False,
# 			  help = "put text into nodes (default: use \\pgftext, support rotation)")
options, args = op.parse_args()

if options.splines not in ("lines", "plot"):
	op.error("argument of --splines must be either 'lines' or 'plot'")

# FIXME: more natural arguments like
# --pattern = off|on
# --fonts off|type|on
# --splines lines|plot

# --------------------------------------------------------------------

assert len(args) == 1

c = TikZConverter(fig.File(args[0]), sys.stdout)
c.includeBaseDir = options.baseDir
c.scale *= options.scale
c.detectNodes = options.detectNodes
c.connectTolerance = options.detectNodes and fig.unitCM / 10. # FIXME
#c.useTextNodes = options.textNodes
c.textAnchor = options.textAnchor
if options.nofonts:
	c.fontMag = 0
c.logicalThickness = not options.appearance
c.optimalAppearance = options.appearance
c.defineYAxis = options.defineYAxis
c.splinesAsPolylines = options.splines == "lines"
c.detectClosing = True # TODO?
c.writePicture()

